DataPerf: Benchmarks for Data-Centric AI Development

Machine learning research has long focused on models rather than datasets, and prominent datasets are used for common ML tasks without regard to the breadth, difficulty, and faithfulness of the underlying problems. Neglecting the fundamental importance of data has given rise to inaccuracy, bias, and fragility in real-world applications, and research is hindered by saturation across existing dataset benchmarks. In response, we present DataPerf, a community-led benchmark suite for evaluating ML datasets and data-centric algorithms. We aim to foster innovation in data-centric AI through competition, comparability, and reproducibility. We enable the ML community to iterate on datasets, instead of just architectures, and we provide an open, online platform with multiple rounds of challenges to support this iterative development. The first iteration of DataPerf contains five benchmarks covering a wide spectrum of data-centric techniques, tasks, and modalities in vision, speech, acquisition, debugging, and diffusion prompting, and we support hosting new contributed benchmarks from the community. The benchmarks, online evaluation platform, and baseline implementations are open source, and the MLCommons Association will maintain DataPerf to ensure long-term benefits to academia and industry.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Section~\ref{sec:dataperf} discusses the benchmarks we introduce and Section~\ref{sec:platform} provides an overview of our server platform for benchmark evaluation.}
  \item Did you describe the limitations of your work?
    \answerYes{Section~\ref{sec:dcai} details the complexity in Data-Centric AI benchmarking and Section~\ref{sec:challenges} and Fig.~\ref{fig:dataperf_pipeline} highlight underserved components in existing benchmarks; our five benchmarks take steps to address these.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Section~\ref{sec:ethics} contains our ethics statement.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{All benchmarks and baselines are open-sourced at \url{https://github.com/MLCommons/dataperf} with code and datasets linked to from \url{https://dataperf.org} and with a snapshot of all key documentation included in the Appendix. }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The GitHub readmes for each baseline implementation provide documentation and all training details for reproducibility.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We only report averages across random seeds in our baselines, as the leaderboards are ranked based on these averages.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In Sec.~\ref{sec:platform} we discuss our serverless architecture and note that benchmark participants are provided with all necessary tools to perform local/offline development and evaluations.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We employ derived datasets and cite them in all relevant sections}
  \item Did you mention the license of the assets?
    \answerNA{We do not redistribute licensed data, so users go through the original data sources.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Participants are informed their usernames are visible on the benchmark evaluation website.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We overview the additional safeguards we provide for potentially offensive content in Sec.~\ref{sec:ethics} and in Appendix~\ref{sec:Appendix:nibbler}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{Adversarial Nibbler uses crowdsourcing and Appendix~\ref{sec:Appendix:nibbler} in the supplementary material contains the instructions and guidelines shared with participants.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> dataperf_org.tex <==
\section{DataPerf}
\label{sec:dataperf}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/overview.pdf}
    \vspace{-0.5cm}
    \caption{Design overview for DataPerf to illustrate the data-centric ML engineering process and the section references for the corresponding DataPerf benchmarks.}
    \label{fig:overview}
\end{figure}

We intend DataPerf to help address the lack of fundamental understanding of how to best engineer ML datasets and the absence of high productivity and efficient open data engineering tools in the machine learning community. DataPerf will make building, maintaining and evaluating datasets easier, cheaper, and more repeatable, regardless of which institution(s) you are affiliated with. Figure~\ref{fig:overview} shows how datasets and models come together during the development of an ML solution using a data-centric ML engineering process and provide section references for the detailed description of DataPerf benchmarks that address specific parts of the process.

DataPerf contains several types of benchmarks, as summarized in Table~\ref{tab:tasks}. Each of the benchmark types is described in more detail in the remainder of this section.

% Please add the following required packages to your document preamble:
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\caption{Benchmark types in DataPerf.}
\label{tab:tasks}
\resizebox{\textwidth}{!}{
\begin{tabular}{   p{\dimexpr 0.2\linewidth-2\tabcolsep} 
                   p{\dimexpr 0.0\linewidth-2\tabcolsep} 
                   p{\dimexpr 0.4\linewidth-2\tabcolsep} 
                   p{\dimexpr 0.4\linewidth-2\tabcolsep}  } \toprule
\multicolumn{2}{l}{\textbf{Benchmark Type}} & \textbf{Benchmark Methodology}                                                                                                                         & \textbf{Benchmark Metric}                                                                                                                                                                             \\\midrule
\multicolumn{2}{l}{Training Dataset}                       & Replace training set with novel training dataset                                                                                              & Accuracy of models trained on novel training dataset                                                                                                                                         \\\midrule
\multicolumn{2}{l}{Test Dataset}                           & Select a fixed number of additional test data from the supplemental data set                                                                  & Number of test datums submitted which are incorrectly labeled by models and correctly labeled by humans, where credit for each item is divided by number of submissions containing that item \\\midrule
\multicolumn{2}{l}{Selection Algorithm}                    & Replace training dataset with subset                                                                                                          & Accuracy of models trained on subset                                                                                                                                                         \\\midrule
\multicolumn{2}{l}{Debugging Algorithm}                    & Identify labeling errors in version of training dataset with some corrupted labels                                                            & Accuracy of trained models after identified labels are corrected                                                                                                                             \\\midrule
\multicolumn{2}{l}{Slicing Algorithm}                      & Divide training dataset into semantically coherent slices                                                                                     & Fraction of data assigned to the correct slice                                                                                                                                               \\\midrule
\multicolumn{2}{l}{Valuation Algorithm}                    & Estimate accuracy improvement from training on dataset A to training on dataset A + dataset B (where B is without labels at time of estimate) & Absolute difference between predicted accuracy and actual accuracy\\\bottomrule
\end{tabular}
}
\end{table}



\subsection{Overview}
We intend DataPerf to help address the lack of fundamental understanding of how to engineer ML datasets and the absence of high productivity and efficient open data engineering tools in the machine learning community to make building, maintaining and evaluating datasets easier, cheaper and more repeatable. Figure 1 shows how datasets and models come together during the development of an ML solution using a data-centric ML engineering process and provide section references for the detailed description of DataPerf benchmarks that address specific parts of the process.


\subsection{Benchmark Types}
\subsubsection{Training Dataset}
\textbf{Purpose:} Generating data, augmenting data, and other data-centric techniques can transform limited datasets into valuable training sets, but finding the right combination of methods can be a painstaking and error-prone process. Each form of data manipulation represents an entire sub-area in the literature and has many nuances. For example, even simple data augmentation techniques like vertical flip can have corner cases (e.g., "6" vs. "9") and may only apply to specific domains (e.g., in medical imaging, "a vertical flip of a mass would still result in a realistic mass \citep{hussain2017differential}"). Using multiple techniques quickly becomes an open-ended problem with a combinatorial set of solutions. The challenge is creating a pipeline of steps that expands a limited dataset into one representative of the real world. This type of benchmark aims to encourage our understanding of how to transform data into a valuable training set.

\textbf{Measures:} Training dataset benchmarks measure a novel training dataset by training various models and measuring the resulting accuracy. In most machine learning competitions, you are asked to build a high-performance model given a fixed dataset. Here we invert the traditional format and ask you to improve a dataset given a fixed model. Submitters are provided with a dataset to improve by applying data-centric techniques such as adding examples representing edge cases and using data augmentation.

\textbf{Metric:} The accuracy of a fixed model(s) trained on the submitted dataset and evaluated on a hidden test set. 

\subsubsection{Test Dataset}

\textbf{Purpose:} Conceptually, a Test Dataset benchmark measures a novel test dataset, or adversarial test data for inclusion in such a dataset, by evaluating if it is (1) labeled incorrectly by a variety of models, (2) labeled correctly by a humans, and (3) novel relative to other existing test data. The purpose of this type of benchmark is to foster innovation in the way we sample data for test sets and build an understanding of how data properties influence ML performance with respect to accuracy, reliability, fairness, diversity, and reproducibility. 

\textbf{Measures:} Test dataset benchmarks measure a set of “adversarial” test data examples. Each participant is given a dataset of candidate data and asked to select a fixed number of “adversarial” examples. Adversarial examples are those for which a standard set of models fail to predict the label correctly. Participants will be allowed to employ any creative strategy, from human-curation to algorithmic data selection/prediction. Initially, only data from the target dataset will be allowed for submission and only for the target list of labels provided. New data, augmented data, or generative approaches will not be allowed.

\textbf{Metric:} The Test Dataset benchmark metric is the sum across the set of examples where human raters verify the label and one or more models fail to identify the label of each such example. The value is the fraction of models that fail to identify the label correctly. In the case of a challenge based on the benchmark, the value is divided by the number of submissions that include the particular example to reward rarer instances.

\subsubsection{Selection Algorithm }

\textbf{Purpose:} Collecting large amounts of data has become straightforward, but turning that data into useful training sets has not. The unprecedented amount of available data in practice holds a wealth of information about the world around us. However, unlocking that value can be cumbersome and resource-hungry. Naively processing the data wastes valuable computational and labeling resources because the data is often redundant and heavily skewed. If we shift the focus to the long-tails, we can save valuable resources while maintaining quality. The challenge is algorithmically identifying and selecting the most informative examples from a dataset to use for training.


\textbf{Measures:} The selection algorithm benchmark evaluates the quality of algorithmic methods for curating datasets (e.g., active learning or core-set selection techniques). Selection algorithms identify the most informative examples from a large dataset. Each algorithm will select, target class, and submit the best possible training data of maximum size (e.g., 1,000 examples) from a dataset for a fixed set of target classes (e.g., 200 examples per class).

\textbf{Metric:} The submitted data will be evaluated by (1) training a fixed set of models, (2) evaluating the resulting models on held-out data, and (3) aggregating the quality scores across models and held-out datasets. The models are fixed and fine-tune pre-computed embeddings to keep the benchmark affordable and focused on data as the primary degree of freedom.

\subsubsection{Data Debugging Algorithm}
\textbf{Purpose:} Training datasets often contain data errors. On one hand, these can be missing values (e.g. NULL values, or values that break functional dependencies such as City->ZIP Code). On the other hand, they can be wrong values (e.g. wrong labels, or noisy features undetectable by simple data validators). Repairing data errors is usually a costly process that often involves human labor. It is therefore useful to manage the tradeoff between the cost of repair and expected benefits. Given a fixed budget B representing the number (or proportion) of data examples that are allowed to be repaired, the challenge is to select a subset of training examples that will give the biggest improvement in the performance of the trained model.

\textbf{Measures:} DataPerf challenges provide a collection of problems, each defined by a set of attributes (e.g. source dataset, type of data error, error distribution across examples, model type etc). For each problem, we provide a labeled training dataset containing artificially injected data errors (following some combination of a random strategy, or rule based, or maybe even manual). If the error type is missing values, for each missing value (designated by NULL), we provide a corresponding set of viable “candidate values”, one of which is the “true” one. Also, this “erroneous dataset” is accompanied by a “repaired dataset” which is used for evaluation but should be hidden from the algorithm. Finally, a labeled validation dataset (used for tuning the algorithm) and a test dataset (used for the final evaluation; should be hidden from the algorithm) are provided.

\textbf{Metric:} After applying the data repairs within the constraints of the budget B, a model (specified by the appropriate problem attribute) is trained and its performance (e.g. accuracy) is evaluated. The same process is repeated for the initial erroneous dataset and the fully repaired dataset, which allows to establish the min and max bars of model performance (denoted perf\_err and perf\_rep). Finally, the score of the data debugging algorithm is expressed as the amount of “performance gap closed”, that is, (perf\_alg - perf\_err) / (perf\_rep - perf\_err).

\subsubsection{Valuation Algorithm}
\textbf{Purpose:} The purpose of this type of benchmark is to foster innovation in dataset creation through data acquisition. Conceptually, there is a data market, with data acquirers and data providers making transactions at a dataset granularity. Datasets can be labeled or unlabeled. For this challenge, we focus on an unlabeled dataset. This challenge aims to help data acquirers estimate the incremental value of an unlabeled dataset, prior to acquisition and labeling, against an existing labeled dataset.

We assume the data acquirer already has a local dataset ($D_A$), which it uses to train its local model. However, this model is not good enough and the acquirer wants to acquire more data examples to improve their model. There is a data provider with an unlabeled dataset ($D_B$). The data acquirer needs a lightweight algorithm to estimate the value of the entire dataset before acquisition and labeling. We assume data acquirers and providers are connected through a trusted, auditable computation infrastructure, which has access to providers' and acquirers' data. 

\textbf{Measures:} The DataPerf Valuation benchmark measures the quality of an algorithm that estimates the relative value of using a new dataset $D_B$  along with an existing dataset $D_A$ with respect to a test set $D_{test}$ and $\text{Model_M}$, where $D_B$ does not have labels at the time of the estimate. Participants will be provided the labeled dataset $D_A$ and unlabeled dataset $D_B$, a $Model_M$, and a test set $D_{test}$ to evaluate their algorithm. Participants will be allowed to employ any creative strategy possible, from algorithmic labeling of the unlabeled dataset to unsupervised learning. However, introduction of new data, trained models, or manual labeling of the dataset is not allowed. 

\textbf{Metric:} The base metric is the absolute difference between estimated accuracy $Acc’(D_A + D_B)$ to the true accuracy $Acc(D_A + D_B)$  of a model trained on the union of the two datasets. The true accuracy will be calculated with the true labels during the evaluation of the participants’ algorithms. For more thorough evaluation, the full metric is the root mean squared error across a range of such problems.

\subsubsection{Slice Discovery Algorithm}
\textbf{Purpose:} Machine learning models that achieve high overall accuracy often make systematic errors on important subgroups (or slices) of data. For instance, models trained to detect collapsed lungs in chest X-rays have been shown to make predictions based on the presence of chest drains, a device typically used during treatment. As a result, these models frequently make prediction errors on cases without chest drains, a critical data slice where false negative predictions could be life-threatening. Identifying underperforming slices is challenging when working with high-dimensional inputs (e.g. images, audio) where data slices are often unlabeled. This benchmark evaluates automated slice discovery algorithms that mine unstructured data for underperforming slices.  

\textbf{Measures:} The DataPerf Slice Discovery benchmark consists of a large set of slice discovery problems. Each problem includes (1) a labeled dataset, (2) a model trained on that dataset, and (3) ground truth slice annotations for one or more slices on which the model makes systematic errors. For example, one slice discovery problem in the benchmark includes a dataset of images with binary labels for the class ``vehicle'', a model trained to detect vehicles, and labels for a critical data slice, ``mopeds'', on which the model underperforms. Participants are asked to submit algorithms that given the (1) dataset and (2) model can automatically identify the underperforming (3) slice. An algorithm may output up to five slices, each specified as ranking over the examples in the dataset.

\textbf{Metric:}  When using slice discovery algorithms, practitioners typically inspect the top-k examples in a predicted slice to understand what concept the slice corresponds. Our primary metric, the maximum precision-at-k between a predicted slice and the ground truth slice, aligns well with this use case. Maximum precision-at-k is computed for each problem in the benchmark. Each slice discovery algorithm gets a single score for comparisons and leaderboards: the average maximum precision-at-k across the problems. 

\subsection{Suite: Benchmark Types x Tasks}

We define the DataPerf Benchmark Suite as a cross-product of benchmark types and specific ML tasks to measure the datasets or algorithms under test. Specifically, the initial version of DataPerf uses the following tasks:

\textbf{Image Classification:} The Image Classification task involves labeling images from Open Images. Open Images was chosen because of its large size and permissive license.

\textbf{Roman Numeral OCR:} The Roman Numeral OCR task identifies hand-written roman numerals. Roman numerals were chosen because the limited domain makes it easy to generate novel data, and there is no major existing dataset that could be submitted to the training set benchmark.

\textbf{Keyword Identification:} The keyword identification task involves labeling short speech utterances with the spoken work.

\textbf{NLP:} The Natural Language Processing task encompasses five subtasks from the Dynabench Platform \citep{kiela2021dynabench}, including hate speech detection \citep{vidgen-etal-2021-learning}, natural language inference \citep{nie-etal-2020-adversarial}, question answering \citep{bartolo-etal-2020-beat}, sentiment analysis \citep{potts-etal-2021-dynasent}, and visual question answering \citep{sheng2021human}. % All of these datasets were collected adversarially (see also \citep{jia-liang-2017-adversarial})

We use this benchmark matrix for three reasons. First, each column embodies a data ratchet for a specific problem in the form of a training set benchmark and a test set benchmark. Second, the same algorithm can be submitted to all benchmarks in the same row for algorithmic benchmarks to demonstrate generality. Third, pragmatically, rules and infrastructure developed to support one benchmark may be leveraged for other challenges. Fourth, the Dynabench platform has made initial strides towards improving leaderboard culture, with leaderboard infrastructure that can be dynamically expanded or adjusted. 

\subsection{Competition: Leaderboards + Challenges}
We plan leaderboards and challenges based on the DataPerf benchmarks to encourage constructive competition, identify best-of-breed ideas, and inspire the next generation of concepts for building and optimizing datasets. A leaderboard is a public summary of benchmark results. Leaderboards help to identify state-of-the-art approaches quickly. A challenge is a public contest to achieve the best result(s) on a leaderboard in a fixed period of time. Challenges motivate rapid progress in developing new approaches through recognition, awards, and/or prizes. We are interested in benchmarks related to the quality of the datasets and the algorithms for working with datasets. We will host the leaderboard and challenges on an augmented Dynabench system supported by the MLCommons Association.



==> divisions.tex <==
\section{Open and Closed Divisions}

DataPerf provides two submission categories for challenge participants: the open and closed divisions. In the open division, we look for creative ideas that use any algorithm to tackle a problem, including those that involve a manual component (i.e., a human in the loop).
In the closed division, we seek to ensure rigorous reproducibility and equitable comparison of similar approaches. For instance, open-division submitters to the speech selection algorithm challenge (Section\ref{sec:speech}) must describe their developed technique and provide their training set. We then evaluate the set's quality. In the closed division, on the other hand, participants must submit a description of their technique, the training set they created, and the code they used to construct the training set. We then review the results and rate the training set. In addition, we execute the submitted code to ensure it creates the specified training set. Therefore, the closed division prohibits solutions with a manual component. These two categories allow us to accommodate submitters who wish to avoid divulging their methods because they contain proprietary logic; other open-source developers, however, may wish to share their solutions and facilitate rapid adoption.
DataPerf currently only supports submissions to the open division, but future submissions rounds will include closed division submissions.

==> platform.tex <==
\section{Evaluation Platform}\label{sec:platform}
DataPerf provides an online platform where benchmark participants can submit their solutions for evaluation, and a working group which invites members in academia and industry to propose new data-centric challenges for inclusion in the DataPerf suite. 
%This platform supports functionality for hosting datasets, registering users, collecting and validating submissions, and enabling both algorithmic and human-in-the-loop evaluations of submissions. 
%A task can be run over multiple annotation rounds over which the models in the loop may be updated and improved.
%The goal of our online platform is to make building, maintaining and evaluating datasets easier, cheaper and more repeatable. 
The DataPerf benchmarks, evaluation tools, leaderboards, and documentation are hosted in an online platform called Dynabench\footnote{\url{https://dynabench.org/}}\citep{kiela2021dynabench}, which allows benchmark participants to submit, evaluate, and compare solutions for all data-centric benchmarks defined in Sec.~\ref{sec:dataperf}. 
% Dynabench initially began as an effort to support dynamic data collection and evaluation for NLP tasks\citep{kiela2021dynabench}, and to address static dataset issues such as saturation, susceptibility to overfitting, and exploitable annotator artifacts. 

%to improve ML through benchmarks, open data and recommendations. 
% We detail the DataPerf-led contributions to Dynabench in the remainder of this section.


DataPerf introduces three key extensions to the Dynabench codebase to support data-centric benchmarks: (1) We add support for a wide variety of submission artifacts, such as training subsets, priority values/orderings, and purchase strategies. Future benchmark authors can contribute customized, modular submission pipelines for different submission artifact types following one of the five examples in Section~\ref{sec:dataperf}. Users can also submit fully containerized systems as artifacts, such as in the debugging challenge.
(2) To support a diverse set of evaluation algorithms and scoring metrics, we develop modular software adaptors to allow for running custom benchmark evaluation tools and displaying or querying scores in Dynabench's online leaderboards. 
% Each , for the Adversarial Nibbler challenge, new logic to communicate with API's from OpenAI and Midjourney was developed, as well as the architecture to support text-to-image benchmarks. Likewise, both speech and vision selection as well as data acquisition underwent enhancements in order to guarantee they would run smoothly in the platform. This meant creating optimizations throughout different stages such as dataset loading as well as actual evaluation, and testing multiple deployment strategies to balance between costs and efficiency. 
(3) In order to prioritize scalability, DataPerf implements a serverless deployment model, allowing it to dynamically scale its resources based on demand, ensuring optimal performance and efficient resource allocation. With this model, the platform can automatically scale with the growth of the benchmark suite and the number of participants.
The NLP-focused original codebase was modularized to provide extensible architectural support for the specific needs of individual challenges. 
For example, the Adversarial Nibbler challenge requires API support for multiple generative AI providers. 
% For speech and vision selection and data acquisition, performance optimizations were implemented on the dataset loading stages to guarantee they would run smoothly in the platform and limit compute costs. 
These improvements to Dynabench ensure DataPerf can easily and cheaply scale with the number of participants and accommodate future data-centric benchmarks from the community. 
All DataPerf challenges, with the exception of Adversarial Nibbler (due to its use of licensed APIs), additionally offer offline evaluation scripts, enabling submitters to iterate on their solution before submitting it to Dynabench. This reduces the load on Dynabench's servers and further improves the scalability of DataPerf.
% Dynabench supports the ability for researchers in academia and industry to propose new data-centric benchmarks for inclusion into DataPerf through an online tool, leveraging the MLCommons evaluation infrastructure. As an open-source server platform\footnote{\url{https://github.com/mlcommons/dynabench}}, users can additionally choose to self-host benchmarks independent of the MLCommons infrastructure. 

The DataPerf benchmarks and the Dynabench platform are open-source, and are hosted and maintained by the MLCommons Association\footnote{\url{https://www.mlcommons.org/}}, a nonprofit organization supported by more than 50 member companies and academics, ensuring long-term availability and benefit to the community.


%MLCommons hosts the MLPerf benchmark suites~\citep{mlperf-training,mlperf-inference}, which emerged from a collaboration between academia and industry to allow fair and relevant ML-system comparisons. Building on this momentum, we want to enable similar progress in ML datasets.

%Over time, DataPerf is intended to extend to cover several other benchmarks types. 
% Finally, given the diversity of the individual challenges, each challenge owner can customize the 

% A crucial addition was the development of a feature that enables the hosting of challenge-specific documentation. This enhancement allows task owners to include information relevant to each challenge, providing participants with context when benchmarking their own artifacts. Likewise, Dynabench is still working on the implementation of communities which will provide a collaborative space for participants, task owners and researchers to engage in discussions and exchange ideas.  (\textcolor{red}{SHOULD WE SPECIFY THAT THIS IS STILL A WORK IN PROGRESS?}). Finally, in the implementation of the Adversarial Nibbler, significant efforts were dedicated towards refactoring the adversarial data collection interface. This involved an overhaul of the existing architecture to accommodate the unique requirements of the challenge. The primary objective was to develop a flexible and reusable framework that would enable new task owners to leverage the components created for this specific challenge. 

    
